Gold Seeker: Information Gain from Policy Distributions for Goal-oriented Vision-and-Langauge Reasoning

As Computer Vision moves from a passive analysis of pixels to active analysis of semantics, the breadth of information algorithms need to reason over has expanded significantly. One of the key challenges in this vein is the ability to identify the information required to make a decision, and select an action that will recover it. We propose a reinforcement-learning approach that maintains a distribution over its internal information, thus explicitly representing the ambiguity in what it knows, and needs to know, towards achieving its goal. Potential actions are then generated according to this distribution. For each potential action a distribution of the expected outcomes is calculated, and the value of the potential information gain assessed. The action taken is that which maximizes the potential information gain. We demonstrate this approach applied to two vision-and-language problems that have attracted significant recent interest, visual dialog and visual query generation. In both cases, the method actively selects actions that will best reduce its internal uncertainty and outperforms its competitors in achieving the goal of the challenge.

==> rel.tex <==

\section{Related work}
%AOur work focus on addressing a series problems labelled Goal-oriented Vision-and-Language Tasks, and in this section, we thus first give a review of previous work in this area. 
%A Especially, we review the related work on goal-oriented visual dialog and compositional VQA. Since our model is a reinforcement learning (RL) based method, we also list the RL work on vision-and-language as our related works and discuss them in the Sec. \ref{rel:el}. We finally review works is intrinsic rewards, which we also adapted in our model.
%A\subsection{Goal-oriented Vision-and-Language Tasks}
\paragraph{Goal-oriented Visual Dialog}
Visual dialog is a recently proposed vision-and-language task that began with image captioning \cite{vinyals2014show,Karpathy2014deepvs,wu2015image} and, includes visual question answering \cite{antol2015vqa,ren2015image,wu2015ask}. Das \etal \cite{das2016visual} proposed a visual dialogue task that requires an agent to engage in conversation with a human centred on the content of a given image.
%Dialogue generation \cite{li2016deep,li2017adversarial,sordoni2015neural}
%has been studied for many years in the NLP literature, and has leaded
%to many applications. The dialogue generation is typically viewed
%as a Seq2Seq problem, or formulated as a statistical machine translation
%problem \cite{ritter2011data,sordoni2015neural}. Recently, the dialogue
%system has been extended to the visual domain. For example, 
%Das \etal \cite{das2016visual} proposed a visual dialogue task that allows
%a machine to engage in conversation with a human centred on the content of a given image.
%Goal-oriented visual dialog demands to understand a user request and complete a related
%task with a clear goal within a limited number of dialog turns. To achieve the goal, the agent needs to seek more information by asking proper questions.
Das \etal \cite{das2017learning} establish two reinforcement learning based agents corresponding to question and answer generation respectively, to finally locate an unseen image from a set of images. The question agent predicts the feature representation of the image and the reward function is given by measuring how close the representation is compared to the true feature.  De Vries
\etal \cite{guesswhat_game} propose a Guess-What game dataset,
where one person asks questions about an image to guess which object
has been selected, and the second person answers questions. Lee \etal \cite{lee2018answerer} adapt the information theoretic approach which allows a questioner to ask appropriate consecutive questions in the GuessWhat setting. 
%Zhang \etal \cite{zhang2018goal} carefully designed three rewards to encourage an agent to ask more informative questions. Our proposed `seeker' model is used as a question generator to generate better questions to query information.

\begin{comment}
Early goal-oriented dialogue systems \cite{wang2013simple,young2013pomdp}
model conversation as a partially observable Markov Decision Processes
(MDP) with many hand-crafted features for the state and action space
representations, which restricts their use to narrow domains. Bordes
\etal \cite{bordes2016learning} propose a goal-oriented dialogue
testbed that requires a user chat with a bot to book a table at a
restaurant. In contrast to previous work that all assume a cooperative
setting, Lewis \etal \cite{dealornodeal} provide a large dataset
of human-human negotiations on a multi-issue bargaining task, where
agents who cannot observe each other's reward functions must reach
an agreement (or a deal) via natural language dialogue. In other words,
the agents have adversarial goals. In visual dialogue, De Vries
\etal \cite{guesswhat_game} propose a Guess-What game dataset,
where one person asks questions about an image to guess which object
has been selected, and the second person answers questions as yes/no/NA.
In our paper, we propose an uncertainty-aware information-seeking
dialogue generator that is able to work on both visual and language
based dialogue systems, with either cooperative or adversarial
goals.
\end{comment}

\vspace{-10pt}
\paragraph{Compositional VQA}
Visual question answering is an AI-complete task that requires a model to answer image-related questions. An increasingly popular research direction in this area is to consider modular architectures. This approach involves connecting distinct modules designed for specific desired capabilities such as memory or specific types of reasoning. Neural Module Networks (NMNs) were introduced by Andreas \etal in \cite{andreas2016learning,andreas2015deep}. 
There the question parse tree is turned into an assembly of modules from a predefined set, which are then used to answer the question. Johnson \etal \cite{clevr} propose a Compositional Language and Elementary Visual Reasoning (CLEVR) dataset that allows the question to be transferred to a sequence of functional problems, which can be further used to query information for the structured scene representation to help to answer the question. In this paper, our  `seeker' model is used as a program generator to generate functional programs from questions.


%A\subsection{Reinforcement Learning}
%A\label{rel:el}
\vspace{-10pt}
\paragraph{RL in Vision-and-Language}
Reinforcement learning (RL) \cite{kaelbling1996reinforcement,sutton1998reinforcement} has been adopted in several vision-and-language problems, including image captioning~\cite{liu2016optimization,ren2017deep,rennie2016self}, VQA~ \cite{andreas2016learning,hu2017learning,zhuknowledge}, and aforementioned visual dialogue system ~\cite{das2017learning,lu2017best} \etc. Recently, some works \cite{asghar2016online,su2016continuously}
make an effort to integrate the Seq2Seq model and RL. RL has also
been widely used to improve dialogue managers, which manage transitions
between dialogue states \cite{singh2002optimizing,pietquin2011sample}. Most recently, Wu~\etal \cite{wu2017you} combines reinforcement learning and generative adversarial networks (GANs) to generate more human-like dialogues. However, nearly all of the methods use a single policy that translates the input sequence to the output while disregarding the strategic diversity needed. In our work, we instead maintain a distribution of policies. And The posterior in our RL framework is updated based on its evaluation of how much it gains towards achieving its goal once the additional information is obtained. Our agent is capable of considering various strategies for obtaining further information, analogous to human contemplation of various ways to ask a question.

%Reinforcement learning (RL) has been applied in many dialogue settings.
%Li \etal \cite{li2016deep} simulate two virtual agents and hand-craft
%three rewards (informativity, coherence and ease of answering) to
%train the response generation model. Recently, some works \cite{asghar2016online,su2016continuously}
%make an effort to integrate the Seq2Seq model and RL. RL has also
%been widely used to improve dialogue managers, which manage transitions
%between dialogue states (\cite{singh2002optimizing,pietquin2011sample}).

%In visual dialogue, Das \etal \cite{das2016visual} use reinforcement
%learning to improve cooperative bot-bot dialogues. Wu \etal \cite{wu2017you}
%combines reinforcement learning and generative adversarial networks
%(GANs) to generate more human-like dialogues. While choosing the optimal
%action is studied in the general RL context such as in multi-armed
%bandit settings \cite{rl_intro,ucb}, it is under-explored in
%dialogue generation.

%Recently, Lipton \etal \cite{lipton2017bbq} proposed a Bayes-by-Backprop
%Q-network (BBQ-network) to approximate the Q-function and the uncertainty
%in its approximation. It encourages a dialogue agent to explore state-action
%regions in which the agent is relatively uncertain in action selection.
%However, BBQ-network only uses Thompson sampling to model the distribution
%of rewards for the words in a Bayesian manner and ignores the uncertainty
%in the estimators (most importantly in the Q function). This can lead
%to very uncertain decisions about confident actions or vice versa.
%Ours, on the other hand, models both the uncertainty in the actions
%(i.e. word choices) and the estimators by directly incorporating the
%variance in the sampling procedure. We provide a theoretical justification
%for the selection which is guaranteed to minimize regret. 
%A*** this sounds a lot like the other paper, it should be different


\vspace{-10pt}
\paragraph{Intrinsic rewards}
The notation of intrinsic reward which focuses of the rewards beyond what is gained from the environment has recently gained attention in the RL community. These rewards are motivated by sparse nature of the environment rewards and a need for better exploration.
For example, curiosity \cite{curiosity} is one such intrinsic reward mechanism within which agents are encouraged to visit new states.  This idea has been extended to employ Bayesian methods to learn the expected improvement of the policy for taking an action \cite{vime,bayesian_surprise,optimal_bayesian}.
We use the expected gain from the answer in the vision-language task as an intrinsic reward to improve our model. 
Nevertheless, our approach is flexible enough that can be easily integrated with any of such additional intrinsic rewards.

